HI-GAN: Hierarchical Inpainting GAN with Auxiliary Inputs for Combined RGB and Depth Inpainting

Inpainting involves filling in missing pixels or areas in an image, a crucial technique employed in Mixed Reality environments for various applications, particularly in Diminished Reality (DR) where content is removed from a user's visual environment. Existing methods rely on digital replacement techniques which necessitate multiple cameras and incur high costs. AR devices and smartphones use ToF depth sensors to capture scene depth maps aligned with RGB images. Despite speed and affordability, ToF cameras create imperfect depth maps with missing pixels. To address the above challenges, we propose Hierarchical Inpainting GAN (HI-GAN), a novel approach comprising three GANs in a hierarchical fashion for RGBD inpainting. EdgeGAN and LabelGAN inpaint masked edge and segmentation label images respectively, while CombinedRGBD-GAN combines their latent representation outputs and performs RGB and Depth inpainting. Edge images and particularly segmentation label images as auxiliary inputs significantly enhance inpainting performance by complementary context and hierarchical optimization. We believe we make the first attempt to incorporate label images into inpainting process.Unlike previous approaches requiring multiple sequential models and separate outputs, our work operates in an end-to-end manner, training all three models simultaneously and hierarchically. Specifically, EdgeGAN and LabelGAN are first optimized separately and further optimized inside CombinedRGBD-GAN to enhance inpainting quality. Experiments demonstrate that HI-GAN works seamlessly and achieves overall superior performance compared with existing approaches.

==> 4model_original.tex <==


\subsection{Generative Adversarial Networks}



\section{Methodology}
We design a novel model called Hierarchical-GAN model which comprises of 3 GAN models working together for RGB and Depth image inpainting. The first GAN model or the EdgeGAN is used for inpainting edge images with missing pixels, the second GAN model or the LabelGAN is used for inpainting semantic segmetation label images. The third and final GAN model or the CombinedGAN model is used for inpainting RGB and Depth images by taking the help from the EdgeGAN and the LabelGAN model.  The EdgeGAN and the LabelGAN model provide edge and semantic segmentation information to the CombinedGAN model which improved RGB and Depth inpaiting. To make the EdgeGAN and LabelGAN be a more powerful regularizer we not only optimize them when training them but we also optimize them once again when we are training the combined model. Both of the EdgeGAN and LabelGAN model comprises of generator and discriminator respectively. The combined model also consists of a generator and discriminator with a fusion module to combine the rgb, depth, edge and label information. Our model can be trained in an end to end manner with the input being rgb, depth, edge, segmentation and mask images and the output being rgb and depth images with no missing pixels. The EdgeGAN and LabelGAN act a regularizer for the CombinedGAN model assisting the model to learn information from edge and label images by trying to fill in the missing pixels in the edge and label images respectively. 
Our novel idea of optimizing the EdgeGAN and LabelGAN model inside the combined GAN model makes the EdgeGAN and LabelGAN model quite powerful on their own as they are optimized twice for each optimization step of the Combined model. The EdgeGAN and LabelGAN model encoder are  thus able to learn features and when combined with the RGB and Depth encoder produce better results that some of the well established models for image inpainting.

\subsection{Network Architecture}
In this section we describe the models that we develop for RGBD inpainting.

\subsubsection{EdgeGAN and LabelGAN}
Our model uses 3 GAN architectures which work together for RGBD inpainting. We first decribe the first and the second GAN model which are the EdgeGAN and the LabelGAN models. These have a familiar GAN architecture with a Generator and Discriminator. We will denote the generator for the EdgeModel to be $G_E$ and for the LabelGAN to be $G_L$. Similarly for the discriminator we have $D_E$ and $D_L$. The generator for both the models have an encoder ($Encoder_{Edge}$, $Encoder_{Label}$) and decoder ($Decoder_{Edge}$, $Decoder_{Label}$) structure which comprise of gated convolution, gated residual blocks, instance normalization and ReLU activations. The discriminator for the EdgeGAN and LabelGAN is a patchGAN\cite{} based discriminator with spectral normalization and LeakyReLU activatations. Figure shows the structure of the EdgeGAN or the LabelGAN model. The input to the EdgeGAN and the LabelGAN are edge and label images along with binary masks to represent missing pixels and the output of both the models are edge and label images with no missing pixels respectively. 
(explain why we do this?)
Our CombinedRGBD-GAN model is called hierarchical GAN because we not only optimize the EdgeGAN and the LabelGAN model when we train them but we also optimize them again inside the CombinedRGBD-GAN model. This makes the EdgeGAN and the LabelGAN model to act as powerful regularizer and help guide the generation of the inpainted RGBD image. 

% \paragraph{Loss Function:} 
% The loss functions used to train the EdgeGAN and LabelGAN are Adversarial Loss and Feature Matching loss or FM loss. We also have hyperparameters which control how much each loss term contributes to the overall loss value. 
% The loss function for the EdgeGAN and LabelGAN is shown below \textcolor{red}{(fill the adversarial and fm by formula)}:

% \begin{gather}
%     \mathcal{L}_e = \lambda^e_a \mathcal{L}^e_a + \lambda^e_{fm} \mathcal{L}^e_{fm}  \\
%     \mathcal{L}_l = \lambda^l_a \mathcal{L}^l_a + \lambda^l_{fm} \mathcal{L}^l_{fm} 
% \end{gather}

\subsubsection{CombinedRGBD-GAN}
The third GAN model is the CombinedRGBD-GAN model which also has a generator and discriminator architecture but it also uses the output from the EdgeGAN and LabelGAN encoder to boost its performance. First we have an RGB encoder $Encoder_{RGB}$ module which takes in as input masked RGB images, second we have a Depth encoder $Encoder_{Depth}$ module which takes in as input masked Depth images, third we take the input from the encoder module of the EdgeGAN model or the $Encoder_{Edge}$, fourth we take the encoder output of the LabelGAN model or the $Encoder_{Label}$ and then finally we have a fusion decoder $Decoder_{Fusion}$ which combines all of the above inputs and gives us the final RGB plus depth image with no missing pixels. The $Encoder_{RGB}$ and $Encoder_{Depth}$ consists of gated convolutions with instance normalization and ReLU activations along with gated residual blocks to extract relevant information from the masked rgb and depth images. The $Decoder_{Fusion}$ consists of gated upsampling convolutions with instance normalization and relu activations and combines the features from all the 4 inputs to get the final RGBD image with no missing pixels. To evaluate the predicted image we have a patchGAN based discriminator with spectral normalization and LeakyReLU activations. 

\subsection{Optimization}
The loss functions used to train the EdgeGAN and LabelGAN are Adversarial Loss and Feature Matching loss or FM loss. We also have hyperparameters which control how much each loss term contributes to the overall loss value. 
The loss function for the EdgeGAN and LabelGAN is shown below \textcolor{red}{(fill the adversarial and fm by formula)}:

\begin{gather}
    \mathcal{L}_e = \lambda^e_a \mathcal{L}^e_a + \lambda^e_{fm} \mathcal{L}^e_{fm}  \\
    \mathcal{L}_l = \lambda^l_a \mathcal{L}^l_a + \lambda^l_{fm} \mathcal{L}^l_{fm} 
\end{gather}


The loss functions used to train the CombinedRGBD-GAN consists of adversarial loss, feature matching loss, perceptual loss and style loss. The hyperparameters which control how much each loss term contributes to the overall loss value. 
The loss function for the CombinedRGBD-GAN is shown below  \textcolor{red}{(fill the adversarial and fm by formula)}:
\begin{gather}
    \mathcal{L}_c = \gamma_a \mathcal{L}_a + \gamma_{fm} \mathcal{L}_{fm} + \gamma_p \mathcal{L}_p + \gamma_s \mathcal{L}_s
\end{gather}

The combined loss function for the EdgeGAN, LabelGAN and the combined can be given as:

\begin{gather}
    \mathcal{L} = \eta_e \mathcal{L}_e + \eta_l \mathcal{L}_l + \eta_c \mathcal{L}_c 
\end{gather}

